Quantifying Uncertainty in Aggregate Queries over Integrated Datasets

Data integration is a notoriously difficult and heuristic-driven process, especially when ground-truth data are not readily available. This paper presents a measure of uncertainty by providing maximal and minimal ranges of a query outcome in two-table, one-to-many data integration workflows. Users can use these query results to guide a search through different matching parameters, similarity metrics, and constraints. Even though there are exponentially many such matchings, we show that in appropriately constrained circumstances that this result range can be calculated in polynomial time with bipartite graph matching. We evaluate this on real-world datasets and synthetic datasets, and find that uncertainty estimates are more robust when a graph-matching based approach is used for data integration.

==> old.tex <==
To summarize our results, we focus on enumeration queries, SUM/COUNT with predicates, and show that the 1-to-k matching can be solved in polynomial time with Hungarian Algorithm used in Bipartite Graph Matching. On the other hand, the m-to-k matching is significantly harder both in formulation and in solution. One first has to define a consistency requirement over the matching that all m corresponding entities in one table match to the same k in the other table. This leads to a combinatorial number of possibilities and makes the problem computationally hard in general. We discuss special cases (that may happen frequently in practice) where the complexity is much lower.

\section{One-to-One Result Intervals}
To understand how the basic algorithm works, let's consider the one-to-one case.

\subsection{1 to 1 Matching}
The 1-1 matching entails a rather straightforward algorithm as its solution follows the balanced assignment problem solution directly. The 1-1 matching expectation suggests that such entity resolution can be viewed as a graph matching problem. Assume that the edge set $E_1 \times E_2$ has vertices $V_1 \times V_2$ to form a bipartite graph. The edges are drawn according to whether the element from the first table and the element from the second table fulfills the similarity threshold. Then, the weights of the edges are computed according to the target aggregate query. In the case of SUM, for instance, the value assigned to weight of the edge is the sum of the target aggregate query variable for the respective vertices of that edge. At this point, the Hungarian algorithm is applied to the bipartite graph. Achieving a matching $M$ is a task of picking the highest outcome while accounting for overall connections using the Hungarian algorithm assuming that the similarity metric used here approximate the likelihood of a match well. A Matching $M$ would naturally be constrained to be 1 to 1 following directly from the nature of the Hungarian algorithm. Note here that the similarity metric here can be changed depending on what similarity metric would make sense for certain entity matching.



\section{One-to-Many Result Intervals}

\subsection{Computing the Query Diameter}

First, consider the balanced assignment problem. In this case, the left and right parts of the bipartite graph constructed from sets A (left) and B (right) have equal number of vertices. Then, the hungarian algorithm is applied to end up with a matching that improves along augmenting paths, which involves the process of alternating paths between unmatched vertices. The overall complexity of the Hungarian approach is $O(mn + n^2 log n)$ in the general case, but improves downwards to $O(mn + n^2 log log n)$ when all weights are integers. 	

Now, consider the unbalanced assignment problem. In this setting, assume that the larger set is B, and thus the right part of the bipartite graph constructed using elements in set B have more vertices, b, than the vertices on the left part of the bipartite graph constructed using elements from set A, a. This problem is essentially reduced to the aforementioned balanced assignment problem by adding b - a new vertices to the left part of the graph constructed using elements from set A and connecting them with the members of the right side, the larger part, with dummy edge weights of 0.  As a result, the perfect matching outcome of the graph has size a + b. After this process, the Hungarian algorithm is applied to end up with matchings at the desired number of maximum matchings. The power of the Hungarian algorithm in such assignments, both balanced and unbalanced, is two-fold: it has the fastest runtime of a strongly polynomial algorithm in a matching setting, and it accounts for all the existing possible matches, which proves especially useful in decreasing overestimation of outcome.

\subsection{1-N Matching}

Following from the 1-1 bipartite graph matching logic, let N be the number of maximum matches for a matching problem. 

The user defines a set of constraints, which includes: the 1-n entity resolution problem brings up certain edge cases that are not straightforward. To start, we now have multiple resolutions to handle. In this case, we can still use the bipartite matching algorithm to arrive at an aggregate interval in which the values will take place. The maximal matching can be used to find the maximum value that the observed entity resolution could get. On the other hand, a minimal matching can give the minimum value (i.e. the exact match) for that match. 

In 1-n matching terms, the smaller set (A) denotes the 1’s table, and the larger set (B) denotes the n’s table.  The 1’s table undergoes a data duplication process in which each row is duplicated according to the number of maximum matches, n, inputted by the user. This ensures that we can have at maximum user inputted “n” number of matches in a bipartite setting. The maximum and minimum bipartite matching algorithm results are then used to determine the maximum and minimum bounds of the expected results. 

In entity resolution context, this algorithm translates to the following process. the 1’s table undergoes a data duplication process in which each row is duplicated according to the number of maximum matches inputted by the user. This ensures that we can have at maximum user inputted “n” number of matches in a bipartite setting. The maximum and minimum bipartite matching algorithm results are then used to determine the maximum and minimum bounds of the expected results.

\subsection{Shaping the Query Diameter}

The respective values gained from the results of 1-1 and 1-n matching make up the lower and the upper thresholds of the expected values respectively. This interval would allow the users to have more than just a $95\%$ confidence interval: they would have aggregate bounds to make decisions with more certainty.

\subsection{Competitive Frameworks}

Naive Algorithm. The naive approach evaluates each row of the table that will be matched (1’s table) to the table that contains multiple matches (n’s table). Each matching that passes the similarity threshold is considered as a candidate match and stored. After all matchings are done, the candidate matches are sorted according to maximum objective to minimum objective (i.e. maximum price to minimum price according to above example).  Then, the list of sorted candidate matches are sliced according to the maximum number of matches inputted by the user to get the maximum matches, and the lower bound of the list is used to get the minimum match. 

Random Sampling Algorithm. This approach follows the similar steps to the Naive Algorithm with the difference of generating the number of random samples to be withdrawn from the n’s table. Compared to the Naive algorithm, this approach improves the average computation time significantly depending on the sample number that is inputted by the user. However, what is gained from computation time is sacrificed from the accuracy depending on the type of data that is inputted by the user. 

% ///////////////////////////////////////
% EXAMPLE EXPLANATION HERE
% //////////////////////////////////////

To illustrate the problem at hand, assume we have the following tables. 
\begin{table}
  \caption{Product Inventory of Company A}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Google Product & Price \\
    \midrule
    Adobe premiere pro cs3 & 60.00 \\
    Lego Star Wars Pack I-II & 50.00 \\
    Lego & 15.00 \\
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Product Inventory of Company B}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Amazon Product & Price \\
    \midrule
    Adobe premiere pro cs3 &  10\\
    Adobe premiere pro cs3 academic &  61\\
    Adobe premiere pro cs3 upgrade &  20\\
    Lego Batman & 10\\
    LEGO & 10\\
    Lego StarWars I II Pack & 50\\
    Lego StarWars I II Edition & 5\\
  \bottomrule
\end{tabular}
\end{table}

A user wants to find the exact same product matchings from those being sold at Company A and Company B. However, the Company B's inventory is less organized and thus there are multiple products mapping to the same product that are also found on Company A's inventory, as seen in the tables. A possible way to use this product matching outcome involves a COUNT query. Finding the count of these matched products would enable the user to keep an inventory of how many of the same products the retail company can sell from the Company A and Company B vendors they are working with. This would enable them to keep track of which products sell the most, so that they can keep ordering the best-seller items from Company A and B. 

Another use case of doing product matching entails using a SUM query.  Finding a total sum of same products could help the retail company have data on how to price the similar products they bought from the vendors to reconcile the different prices they have from the products. The user gives a maximum number of matchings to be made from Company A's Products table to Company B's Products table. 

Another use case would be to sum all products that have a mapping from Company A table to Company B table. A representation of this query would be the following: 

The SUM Query that this example solves makes the following calculation from the above 2 tables given max $n=5$ and a similarity metric chosen by the user (less than 0.9 jaccard similarity). 

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{background-figures/bp_background.png}
    \caption{Bipartite Matching Outcomes}
    \label{exp-figure}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{background-figures/pc_background.png}
    \caption{Predicate-Constraint Matching Outcomes}
    \label{exp-figure}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{background-figures/SUM: Max n = 5, True n <= 5_alternative.png}
    \caption{Matching Outcomes with straight line indicating perfect mapping SUM}
    \label{exp-figure}
\end{figure}

\begin{table}
  \caption{Result of Bipartite Max Matching Queries}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Bipartite Max Matching Outcome & SUM \\
    \midrule
    Adobe premiere pro cs3, Adobe premiere pro cs3 & 70\\ 
    Adobe premiere pro cs3, Adobe premiere pro cs3 academic & 121\\
    Adobe premiere pro cs3, Adobe premiere pro cs3 upgrade & 80\\
    Lego Star Wars Pack I-II, Lego StarWars I-II Edition & 55\\
    Lego Star Wars Pack I-II, Lego StarWars I II Pack & 100\\
    Lego, Lego Batman, & 25 \\
    Lego, LEGO & 25 \\
    SUM Query Outcome & 476
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Result of Predicate-Constraint Matching Queries}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Predicate-Constraint Matching Outcome & SUM \\
    \midrule
    Adobe premiere pro cs3 academic, Adobe premiere pro cs3 academic & 122
    Adobe premiere pro cs3 academic, Lego Star Wars I II Pack & 110
    Adobe premiere pro cs3 academic, Adobe premiere pro cs3 upgrade & 80
    Adobe premiere pro cs3 academic, Adobe premiere pro cs3 & 70.0
    Adobe premiere pro cs3 academic, Lego Batman & 70.0
    Lego Star Wars Pack I II, Adobe premiere pro cs3 academic & 111.0
    Lego Star Wars Pack I II, Lego Star Wars I II Pack & 100.0
    Lego Star Wars Pack I II, Adobe premiere pro cs3 upgrade & 70.0
    Lego Star Wars Pack I II, Adobe premiere pro cs3 & 60.0
    Lego Star Wars Pack I II, Lego Batman & 60.0
    Lego, Adobe premiere pro cs3 academic & 76.0
    Lego, Lego Star Wars I II Pack & 65.0
    Lego, Adobe premiere pro cs3 upgrade & 35.0
    Lego, Adobe premiere pro cs3 & 25.0
    Lego, Lego Batman & 25.0
    SUM Query Outcome & 1079
  \bottomrule
\end{tabular}
\end{table}




We will start off this discussion with a numerical example to illustrate just how much more accurate our derived result ranges are than simple alternatives.
Consider a real subset of rows from the Google-Amazon product matching dataset:
\begin{table}[ht]\footnotesize
  \caption{Product Inventory of Company A}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Google Product & Price \\
    \midrule
    Adobe premiere pro cs3 & 60.00 \\
    Lego Star Wars Pack I-II & 50.00 \\
    Lego & 15.00 \\
  \bottomrule
\end{tabular}
  \begin{tabular}{cc}
    \toprule
    Amazon Product & Price \\
    \midrule
    Adobe premiere pro cs3 &  10\\
    Adobe premiere pro cs3 academic &  61\\
    Adobe premiere pro cs3 upgrade &  20\\
    Lego Batman & 10\\
    LEGO & 10\\
    Lego StarWars I II Pack & 50\\
    Lego StarWars I II Edition & 5\\
  \bottomrule
\end{tabular}
\end{table}

A user wants to find the exact same product matchings from those being sold at Company A and Company B. However, the Company B's inventory is less organized and thus there are multiple products mapping to the same product that are also found on Company A's inventory, as seen in the tables. A possible way to use this product matching outcome involves a COUNT query. Finding the count of these matched products would enable the user to keep an inventory of how many of the same products the retail company can sell from the Company A and Company B vendors they are working with. This would enable them to keep track of which products sell the most, so that they can keep ordering the best-seller items from Company A and B. 

Another use case of doing product matching entails using a SUM query over prices.  Finding a total sum of same products could help the retail company have data on how to price the similar products they bought from the vendors to reconcile the different prices they have from the products. The user gives a maximum number of matchings to be made from Company A's Products table to Company B's Products table. 

Another use case would be to sum all products that have a mapping from Company A table to Company B table. A representation of this query would be the following: 

The SUM Query that this example solves makes the following calculation from the above 2 tables given max $n=5$ and a similarity metric chosen by the user (less than 0.9 jaccard similarity). 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.32\linewidth]{figures/practicalexample-graphs/bp_max_match_graph.png}
    \includegraphics[width=0.32\linewidth]{figures/practicalexample-graphs/bp_min_match_graph.png}
    \includegraphics[width=0.32\linewidth]{figures/practicalexample-graphs/sum_outcome_intervals.png}
    \label{exp-figure}
\end{figure*}

\iffalse
\begin{table}[ht!]
  \caption{Result of Bipartite Max Matching Queries}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Bipartite Max Matching Outcome & SUM \\
    \midrule
    Adobe premiere pro cs3, Adobe premiere pro cs3 & 70\\ 
    Adobe premiere pro cs3, Adobe premiere pro cs3 academic & 121\\
    Adobe premiere pro cs3, Adobe premiere pro cs3 upgrade & 80\\
    Lego Star Wars Pack I-II, Lego StarWars I-II Edition & 55\\
    Lego Star Wars Pack I-II, Lego StarWars I II Pack & 100\\
    Lego, Lego Batman, & 25 \\
    Lego, LEGO & 25 \\
    \midrule
    SUM Query Outcome & 476
   % \bottomrule
    \end{tabular}
\end{table}

\begin{table}[ht!]
  \caption{Result of Predicate-Constraint Matching Queries}
  \label{tab:freq}
  \begin{tabular}{cc}
    \toprule
    Predicate-Constraint Matching Outcome & SUM \\
    \midrule
    Adobe academic, Adobe premiere pro cs3 academic & 122 \\
    Adobe academic, Lego SW I II Pack & 110 \\
    Adobe academic, Adobe premiere pro cs3 upgrade & 80 \\
    Adobe academic, Adobe premiere pro cs3 & 70.0 \\
    Adobe academic, Lego Batman & 70.0 \\
    Lego SW Pack I II, Adobe premiere pro cs3 academic & 111.0 \\
    Lego SW Pack I II, Lego SW I II Pack & 100.0 \\
    Lego SW Pack I II, Adobe premiere pro cs3 upgrade & 70.0 \\
    Lego SW Pack I II, Adobe premiere pro cs3 & 60.0 \\
    Lego SW Pack I II, Lego Batman & 60.0 \\
    Lego, Adobe academic & 76.0 \\
    Lego, Lego SW I II Pack & 65.0 \\
    Lego, Adobe premiere pro cs3 upgrade & 35.0 \\
    Lego, Adobe premiere pro cs3 & 25.0 \\
    Lego, Lego Batman & 25.0 \\
    \midrule
    SUM Query Outcome & 1079 \\
   \bottomrule
  \end{tabular}
\end{table}
\fi
